Coverage Centrality Maximization in Undirected Networks

Centrality metrics are among the main tools in social network analysis. Being central for a user of a network leads to several benefits to the user: central users are highly influential and play key roles within the network. Therefore, the optimization problem of increasing the centrality of a network user recently received considerable attention. Given a network and a target user $v$, the centrality maximization problem consists in creating $k$ new links incident to $v$ in such a way that the centrality of $v$ is maximized, according to some centrality metric. Most of the algorithms proposed in the literature are based on showing that a given centrality metric is monotone and submodular with respect to link addition. However, this property does not hold for several shortest-path based centrality metrics if the links are undirected. In this paper we study the centrality maximization problem in undirected networks for one of the most important shortest-path based centrality measures, the coverage centrality. We provide several hardness and approximation results. We first show that the problem cannot be approximated within a factor greater than $1-1/e$, unless $P=NP$, and, under the stronger gap-ETH hypothesis, the problem cannot be approximated within a factor better than $1/n^{o(1)}$, where $n$ is the number of users. We then propose two greedy approximation algorithms, and show that, by suitably combining them, we can guarantee an approximation factor of $\Omega(1/\sqrt{n})$. We experimentally compare the solutions provided by our approximation algorithm with optimal solutions computed by means of an exact IP formulation. We show that our algorithm produces solutions that are very close to the optimum.

==> coveragealg.tex <==
\subsection{Coverage centrality algorithm}
Algorithm~\ref{alg:coverage} computes the coverage centrality of all the nodes in $V$.
It is based on the Brandes algorithm for computing the betweenness centrality~\cite{}.
\subsubsection{Correctness}
 
\subsubsection{Time Complexity}
The algorithm performs two Breadth-First search (BFS) (one forward and one backward) for each node. The complexity of running a single BFS is $O(|V|+|E|)$. Therefore, the overall complexity is $O(|V|2(|V|+|E|))=O(|V||E|)$.
\begin{algorithm2e}[t]
	%     \SetKwInOut{Input}{Input}
	%     \SetKwInOut{Output}{Output}
	%     \Input{$S, X$ }
	%     \Output{$S',X'$}
	$c_v\gets 0$, $\forall v\in V$\;
	\For{$s\in V$}{
		$S\gets \emptyset$\;
		$P[w]\gets \emptyset$, $\forall w\in V$\;
		$d [t]\gets -1$, $\forall t\in V$, $d [s]\gets 0$ \;
		$Q\gets \emptyset$, $Q.push(s)$\;
	    \While{$Q$ not empty}{	
	    	$v\gets Q.pop()$\;
	    	$S.push(v)$\;
	    	\ForEach{$w \in N_v$}{
	    		\If{$d[w]<0$}{
	    			$Q.push(w)$\;
	    			$d[w]\gets d[v] + 1 $\;
	    		}
	    		\If{$d[w]= d[v] + 1 $}{
	    				$P[w].append(v)$\;
	    			}
	    		
		    }
	    
	    }	
	    			

	$\delta [v]\gets \emptyset$, $v\in V$\;
	\While{$S$ not empty}{\label{alg:coverage:while:begin}
		$w\gets S.pop()$\;
		\For{$v \in P[w]$}{
			$\delta [v]\gets \delta [v] \cup \delta [w] \cup \{u\}$\;
		}
		\If{$w\neq s$}{
				$c_w \gets c_w +|\delta [w]|$\; 
		}
		
	}\label{alg:coverage:while:end}
	
}
	\caption{Algorithm for computing coverage centrality}
	\label{alg:coverage}
\end{algorithm2e}

==> old.tex <==

\section{Preliminaries - ranking}

The \emph{ranking} of each node $v$ according to its betweenness centrality is defined as
\begin{equation}
\label{def:rank}
 r_v = |\{u\in V~|~c_u>c_v\}| + 1.
\end{equation}

Note that maximizing the coverage value of a node $v$ does not necessarily lead to maximizing the ranking position of $v$. Therefore, we also consider the problem of finding a set $S$ of arcs incident to node $v$ that maximizes \emph{the increment of the ranking} of $v$ with respect to its original ranking. We denote such an increment as $\rho_v(S)$, that is,
\[
 \rho_v(S) = r_v - r_v(S).
\]
Informally, $\rho(S)$ represents the number of nodes that $v$ ``overtakes'' by adding arcs in $S$ to $G$. Therefore, we define the following optimization problem.
\optproblem{Maximum Ranking Improvement (\MRI)}
{An undirected graph $G=(V,E)$; a vertex $v\in V$; and an integer $k\in\mathbb{N}$}
{A set $S$ of arcs incident to $v$, $S=\{\{u,v\}~|~u\in V\setminus N_v\}$, such that $|S|\leq k$}
{Maximize $\rho_v(S)$}
The corresponding problem in directed graphs is defined similarly with the same limitation as the \MCI problem.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Directed graphs}
\label{sec:directed}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If $G$ is directed, for each node $v$, $N_v^i$ and $N_v^o$ denotes the set of in-neighbors and out-neighbors of $v$, respectively, i.e. $N_v^i=\{u~|~(u,v)\in E\}$ and $N_v^o=\{u~|~(v,u)\in E\}$.


In a directed graph $G$, the \MCI problem is defined similarly, but we assume that the set of edges $S$ to be added must have the same orientation, that is they must be all incoming to $v$ or all outgoing from $v$, that is either $S=\{(u,v)~|~u\in V\setminus N^i_v\}$ or $S=\{(u,v)~|~u\in V\setminus N^o_v\}$.


\subsection{Hardness of approximation}
Martin

\subsection{Approximation algorithm}
\todo{blabla}
We focus on the case in which all the edges to be added are incoming to $v$, that is $S=\{(u,v)~|~u\in V\setminus N^i_v\}$.

\begin{theorem}\label{th:submodularityDirected}
 Function $c_v:V\times V \rightarrow \mathbb{N}$ is monotone and submodular for directed graphs.
\end{theorem}
\begin{proof}
Let us denote by $c_v^{st}(S)$ the indicator function on whether a shortest path from $s$ to $t$ in $G(S)$ passes through $v$, that is:
\[
 c_v^{st}(S) = \left\{
 \begin{array}{ll}
  1 & \mbox{if there exists a shortest path from $s$ to $t$ that passes through $v$ in $G(S)$}\\
  0 & \mbox{otherwise.}
 \end{array}
 \right.
\]
Then, 
\[
c_v(S) = \sum_{\stackrel{(s,t)\in V\times V}{s,t\neq v}}c_v^{st}(S)
\]
Since function $c_v$ is a linear combination of functions $c_v^{st}$, we will show that function $c_v^{st}$ is monotone and submodular.

To show the monotonicity, let us consider a solution $S\subseteq (V\setminus N^i_v)\times \{v\}$ and an edge $(u,v)\not\in E\cup S$. If there exists a shortest path from $s$ to $t$ in $G(S)$ passing through $v$, then $c_v^{st}(S)=1$ and $c_v^{st}(S\cup\{(u,v)\})=1$. Otherwise, $c_v^{st}(S)=0$, while $c_v^{st}(S\cup\{(u,v)\})=1$ if a shortest path from $s$ to $t$ in $G(S\cup \{(u,v)\})$ passes through $v$ and $c_v^{st}(S\cup\{(u,v)\})=0$ otherwise. In any case, $c_v^{st}(S\cup\{(u,v)\})\geq c_v^{st}(S)$.

Let us now consider two solutions $S\subseteq T \subseteq (V\setminus N^i_v)\times \{v\}$ and an edge $(u,v)\not\in E\cup T$, we will show that 
\begin{equation}\label{eq:submodularityDirected}
 c_v^{st}(S\cup\{(u,v)\}) - c_v^{st}(S) \geq  c_v^{st}(T\cup\{(u,v)\}) - c_v^{st}(T). 
\end{equation}

If $c_v^{st}(S) = 1$, then there exists a shortest path from $s$ to $t$ passing through $v$ already in $G(S)$ which is the smaller graph considered. Therefore, the same path exists also in $G(S\cup\{(u,v)\})$, $G(T)$, and $G(T\cup\{(u,v)\})$. Hence, $c_v^{st}(S\cup\{(u,v)\}) = c_v^{st}(T) = c_v^{st}(T\cup\{(u,v)\})  = 1$ and Condition~\eqref{eq:submodularityDirected} holds.

If $c_v^{st}(S) = 0$, we have the following cases.
\begin{itemize}
 \item $c_v^{st}(T) = 1$ In this case there exists shortest path from $s$ to $t$  in $G(T)$ passing through $v$. The same shortest path also exists in $G(T \cup \{(u,v)\})$ and then $c_v^{st}(T\cup\{(u,v)\}) = c_v^{st}(T)$, while, by monotonicity, $c_v^{st}(S\cup\{(u,v)\}) \geq c_v^{st}(S)$.
 \item $c_v^{st}(T) = 0$. In this case, no shortest path  path from $s$ to $t$ in $G(T)$ passes through $v$. Let us consider graph $G(\{(u,v)\})$ in which only edge $(u,v)$ is added. If $c_v^{st}(\{(u,v)\}) = 1$, then there exists shortest path from $s$ to $t$ passing through edge $(u,v)$. The same path exists in $G(S\cup\{(u,v)\})$ and $G(T\cup\{(u,v)\})$, and then $c_v^{st}(S\cup\{(u,v)\}) = c_v^{st}(T\cup\{(u,v)\})  = 1$. Otherwise, no path from $s$ to $t$ passes through edges in $T\cup \{(u,v)\}$ and then $c_v^{st}(S\cup\{(u,v)\}) = c_v^{st}(T\cup\{(u,v)\}) = 0$.
 \end{itemize}
In any of the above cases Condition~\eqref{eq:submodularityDirected} holds.
\end{proof}


\subsection{IP}
(Lorenzo)
\begin{equation*}
\begin{array}{ll@{}l}
\text{Maximize}  & \displaystyle\sum_{\substack{s, t \in V\setminus\{v\}\\u\in V\setminus N_v \cup \{v\}}} y_{stu} &\\
\text{subject to}& \displaystyle\sum_{u\in V\setminus N_v \cup \{v\}}y_{stu}\leq 1, & \mbox{for each } s, t \in V\setminus\{v\}\\
& \displaystyle y_{stu}\leq x_u,& \mbox{for each } s, t \in V\setminus\{v\}$ and $u\in V\setminus N_v \cup \{v\},\label{lp:dir:path}\\
& \displaystyle\sum_{u\in V\setminus N_v\cup \{v\}} x_u \leq k,\\
& \displaystyle x_u,y_{stu}\in\{0,1\},&\mbox{for each }s, t \in V\setminus\{v\}$ and $u,w\in V\setminus N_v \cup \{v\}.
\end{array}
\end{equation*}
The decision variables $x_u$ and $y_{stu}$ specify a solution $S$ of the \MCI\ problem as follows. For any $u \in V\setminus N_v$,
$$x_u=\begin{cases}
1&\mbox{if } \{u,v\}\in S,\\
0 &\mbox{otherwise,}
\end{cases}$$
and, for each $s, t \in V\setminus\{v\}$ and $u\in V\setminus N_v \cup \{v\}$, 
$$y_{stu} =  \begin{cases}
1&\mbox{if a shortest path from } s \mbox{ to } t \mbox{ in } G(\{u,v\}) \mbox{ passes through } v,\\
0 &\mbox{otherwise.}
\end{cases}  $$
Notice that constraints~\ref{lp:und:path} are added in the program only if a shortest path between $s$ and $t$ passes trough $v$ in $G(\{u,v\})$.
\subsection{Experiments}





\section{Old algorithm (flawed analysis)}
It is easy to see that, in the undirected case, the objective function is not submodular and that there are instances of the \MCI problem for which the greedy algorithm has a $O(1/n)$ approximation ratio.
\todo{Show example??} The main problem with the greedy algorithm is that it does not take into account the shortest paths that pass through two of the added edges. In this section, we show how to overcome this limitation and we give an algorithm that guarantees a $O(1/k)$ approximation. The algorithm exploits a solution to a subproblem called Maximum Edge-Coverage Improvement (\MECI), which we show to be approximable to within a $1-\frac{1}{e}$ factor. Before going in the detail of the main algorithm, in the following, we define the \MECI problem and show how to achieve this approximation.

Let $E_{st}$ be the set of edges in a shortest path between $s$ and $t$ in $G$. Given two nodes $u$ and $v$ such that edge $\{u,v\}$ does not belong to $E$, we define the \emph{edge coverage centrality} of $\{u,v\}$ as the number of pairs $(s,t)$ such that edge $\{u,v\}$ is contained in a shortest path from $s$ to $t$ in $G(\{u,v\})$, formally,
\begin{equation}
\label{def:ecc}
 c_{uv} = |\{ (s,t)\in V\times V ~|~ \{u,v\}\in E_{st}(\{u,v\}), u,v\neq s, u,v\neq t \}|.
\end{equation}
The Maximum Edge-Coverage Improvement for a pair $(u,v)$, such that $\{u,v\}\not\in E$, consists in finding a set $S$ of arcs incident to node $v$ that maximizes the number of shortest paths passing through edge $\{u,v\}$ in $G(S\cup\{\{u,v\}\})$, that is $c_{uv}(S\cup\{\{u,v\}\})$ is maximum.

\optproblem{Maximum Edge-Coverage Improvement (\MECI)}
{An undirected graph $G=(V,E)$; a pair of nodes $(u,v)$ such that $\{u,v\}\not\in E$; an integer $k'\in\mathbb{N}$}
{A set $S$ of arcs incident to $v$, $S=\{\{w,v\}~|~w\in V\setminus N_v, w\neq u\}$, such that $|S|\leq k'$}
{Maximize $c_{uv}(S\cup\{\{u,v\}\})$}

Like in the directed \MCI problem, we show that there exists a greedy algorithm that approximates \MECI to within a factor $1-\frac{1}{e}$ by proving that function $c_{uv}$ is monotone and submodular.
\begin{theorem}\label{th:submodularityUndirected}
 Function $c_{uv}:V\times V \rightarrow \mathbb{N}$ is monotone and submodular for undirected graphs.
\end{theorem}
\begin{proof}
 The proof is similar to that of Theorem~\ref{th:submodularityDirected}. Let us denote by $c_{uv}^{st}(S)$ the indicator function on whether a shortest path from $s$ to $t$ in $G(S\cup\{\{u,v\}\})$ passes through edge ${u,v}$, that is:
\[
 c_v^{st}(S) = \left\{
 \begin{array}{ll}
  1 & \mbox{if there exists a shortest path from $s$ to $t$ that passes through edge $\{u,v\}$ in $G(S \cup\{\{u,v\}\})$}\\
  0 & \mbox{otherwise.}
 \end{array}
 \right.
\]
Then, 
\[
c_{uv}(S) = \sum_{\stackrel{(s,t)\in V\times V}{s,t\neq v}}c_{uv}^{st}(S)
\]
Since function $c_v$ is a linear combination of functions $c_{uv}^{st}$, we will show that function $c_v^{st}$ is monotone and submodular.

To show the monotonicity, let us consider a solution $S\subseteq (V\setminus (N_v\cup\{u\}))\times \{v\}$ and an edge $\{w,v\}\not\in E\cup S\cup\{\{u,v\}\}$. 

If there exists a shortest path from $s$ to $t$ in $G(S\cup\{\{u,v\}\})$ passing through $\{u,v\}$, then $c_{uv}^{st}(S)=1$ and $c_v^{st}(S\cup\{(w,v)\})=1$. Otherwise, $c_{uv}^{st}(S)=0$, while $c_{uv}^{st}(S\cup\{(w,v)\})\geq 0$. In any case, $c_{uv}^{st}(S\cup\{\{w,v\}\}) \geq c_{uv}^{st}(S)$.

Let us now consider two solutions $S\subseteq T \subseteq (V\setminus (N_v\cup\{u\}))\times \{v\}$ and an edge $\{w,v\}\not\in E\cup T$, we will show that 
\begin{equation}\label{eq:submodularityUndirected}
 c_{uv}^{st}(S\cup\{\{w,v\}\}) - c_{uv}^{st}(S) \geq  c_{uv}^{st}(T\cup\{\{w,v\}\}) - c_{uv}^{st}(T). 
\end{equation}

If $c_{uv}^{st}(S) = 1$, then there exists a shortest path from $s$ to $t$ passing through $v$ already in $G(S\cup\{\{u,v\}\})$ which is the smaller graph considered. Therefore, the same path exists also in $G(S\cup\{\{u,v\}, \{w,v\}\})$, $G(T\cup\{\{u,v\}\})$, and $G(T\cup\{\{u,v\},\{w,v\}\})$. Hence, $c_{uv}^{st}(S\cup\{\{w,v\}\}) = c_{uv}^{st}(T) = c_{uv}^{st}(T\cup\{\{w,v\}\})  = 1$ and Condition~\eqref{eq:submodularityUndirected} holds.

If $c_{uv}^{st}(S) = 0$, we have the following cases.
\begin{itemize}
 \item $c_{uv}^{st}(T) = 1$ In this case there exists shortest path from $s$ to $t$ in $G(T\cup\{\{u,v\}\})$ passing through edge $\{u,v\}$. The same shortest path also exists in $G(T \cup\{\{u,v\},\{w,v\}\})$ and then $c_{uv}^{st}(T\cup\{\{w,v\}\}) = c_{uv}^{st}(T)$, while, by monotonicity, $c_{uv}^{st}(S\cup\{\{w,v\}\}) \geq c_{uv}^{st}(S)$.
 \item $c_{uv}^{st}(T) = 0$. In this case, no shortest path  path from $s$ to $t$ in $G(T\cup\{\{u,v\}\})$ passes through $\{u,v\}$. Let us consider graph $G(\{\{u,v\}, \{w,v\}\})$ in which only edges $\{u,v\}$ and $\{w,v\}$ are added. If $c_{uv}^{st}(\{\{w,v\}\}) = 1$, then there exists shortest path from $s$ to $t$ passing through edges $\{u,v\}$ and $\{w,v\}$. The same path exists in $G(S\cup\{\{u,v\}, \{w,v\}\})$ and $G(T\cup\{\{u,v\}, \{w,v\}\})$, and then $c_{uv}^{st}(S\cup\{\{w,v\}\}) = c_{uv}^{st}(T\cup\{\{w,v\}\})  = 1$. Otherwise, no path from $s$ to $t$ passes through edge $\{u,v\}$ and one of the edges in $T\cup \{\{w,v\}\}$ and then $c_{uv}^{st}(S\cup\{\{w,v\}\}) = c_{uv}^{st}(T\cup\{\{w,v\}\}) = 0$.
 \end{itemize}
In any of the above cases Condition~\eqref{eq:submodularityUndirected} holds.
\end{proof}

We can now describe our approximation algorithm for the undirected \MCI problem, see Algorithm~\ref{algo:undirected} for the pseudo-code. The algorithm approximately solves, for each $u \not\in N_v$, the \MECI instance defined on $G$, pair $(u,v)$, and $k'=k-1$. For each $u$, let $S_u$ be the solution returned by the greedy algorithm for the \MECI instance related to edge $\{u,v\}$. The algorithm selects, among these solutions, the one that maximizes the objective function of the \MCI problem, that is $S=\arg\max_{u \not\in N_v} c_v(S_u\cup\{\{u,v\}\})$. The idea is that, if $S^*$ is an optimal solution for \MCI, then, among all the tested edges $\{u,v\}$, the algorithm guesses one of the edges of $S^*$ that maximizes the number of pairs $\{s,t\}$ which have a shortest path passing through $v$ in $G(S^*)$. The other $k-1$ edges are found by using an approximate solution for the \MECI problem defined on the guessed first edge.

\begin{algorithm2e}[t]
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$S, X$ }
%     \Output{$S',X'$}
  $S:=\emptyset$\;
  \ForEach{$u \not\in N_v$}
  {
    Solve \MECI on $G$, with pair $(u,v)$ and $k'=k-1$\label{algo:undirected:greedy}\;
    Let $S_u$ be the solution returned\;
    \If{$c_v(S_u\cup\{\{u,v\}\}) > c_v(S)$}
    {
      $S:=S_u\cup\{\{u,v\}\}$\;
    }
  }
  \caption{Approximation algorithm for the undirected case}
  \label{algo:undirected}
\end{algorithm2e}

The next theorem shows that Algorithm~\ref{algo:undirected} guarantees a $O(1/k)$ approximation.
\begin{theorem}
 Algorithm~\ref{algo:undirected} is a $\frac{1}{k}\left(1-\frac{1}{e}\right)$-approximation for \MCI on undirected graphs.
\end{theorem}
\begin{proof}
 Let $S^*$ be an optimal solution for \MCI. Let us sort the elements of $S^*$ in non-increasing order according to their marginal contribution to the objective function, that is, according to the number of pairs covered by each edge. Let $\{u^*,v\}$ be the first edge in such ordering, that is, $\{u^*,v\}$ is the edge of $S^*$ that maximizes the number of pairs $\{s,t\}$ which have a shortest path passing through $v$ in $G(S^*)$. Let us consider the iteration of Algorithm~\ref{algo:undirected} in which node $u^*$ is selected. We have that
 
 \[
    c_v(S)\geq c_v(S_{u^*}\cup\{\{u,v\}\})  \geq c_{u^*v}(S_{u^*}),
 \]
 where the first inequality is due to the minimality of $c_v(S)$ with respect to all $u \not\in N_v$, and the last one is due to the fact that any shortest path passing through edge $\{u^*,v\}$ in $G(S_{u^*}\cup\{\{u,v\}\})$, also passes through node $v$ in the same graph. If $S^*_{u^*}$ is an optimal solution for the \MECI instance defined on graph $G$, pair $(u^*,v)$, and budget $k-1$, thanks to the approximation algorithm used at line~\ref{algo:undirected:greedy} of Algorithm~\ref{algo:undirected}, we have that,
 \[
    c_{u^*v}(S_{u^*}) \geq \left(1-\frac{1}{e}\right) c_{u^*v}(S^*_{u^*}).
 \] 
 By definition of $u^*$, the number of pairs that have a shortest paths that pass through node $v$ in $G(S^*)$ is at most $k$ times the number of pairs that have a shortest paths passing through edge $\{u^*,v\}$ in $G(S^*)$. In other words, $c_v(S^*) \leq k\cdot c_{u^*v}(S^*)$. Moreover, $c_{u^*v}(S^*_{u^*}) \geq c_{u^*v}(S^*)$, since $S^*_{u^*}$ is optimal for the considered \MECI instance. Summing up,
 \[
  c_v(S)\geq \frac{1}{k}\left(1-\frac{1}{e}\right)c_v(S^*).\qedhere
 \]
% 
%  
% %  \geq \left(1-\frac{1}{e}\right) \frac{1}{k} OPT$
%  
%  
\end{proof}
NOTE: Generalize to fixed $M=O(1)$, ($M\leq k$) initial edges would give $\frac{M}{k}\left(1-\frac{1}{e}\right)$.

\section{Sketch of Another Algorithm (worse than the greedy with pairs)}

The following is a sketch for a polynomial time algorithm for MCI that has approximation factor $\left(1-\frac{1}{e}\right)/(k-1)$ if the proof holds. 

For two edges $e = (u,v)$ and $f = (w,v)$, we define $S_{ef}$:
$$S_{ef} = \{ (s,t)\in V\times V ~|~ v\in P_{st} \mbox{ in } G(\{e, f\}), v\neq s, v\neq t \} \enspace .$$
$S_{ef}$ is the set of pairs $(s,t)$ for which there would be a shortest path through $v$ if we added $e$ and $f$ to the graph. We extend the notation so that $S_X$ is referring to the pairs with a shortest path through $v$ if the set of edges $X$ was added. We will also need this simple lemma:
\begin{lemma}\label{lem:union_x_y_z}Consider $y$ sets with $x$ elements in the union. If $Z$ is the union with maximum cardinality of $z$ of the sets then 
$$|Z| \geq \frac{z}{y} \cdot x \enspace .$$
\end{lemma}

\begin{proof}Pick a collection of $z$ sets uniformly at random. The probability that an element is in the union of the sets is at least $\frac{z}{y}$ so the union has expected size $\frac{z}{y} \cdot x$.
\hfill \qed
\end{proof}

The algorithm works as follows:
\begin{enumerate}
  \item Choose $k/2$ sets $S_{ef}$ using the greedy algorithm for maximum coverage in an attempt to maximise the cardinality of their union. Let $P$ be the corresponding set of pairs of edges: $P = \cup_{i=1}^{k/2} \{(e_i, f_i)\}$.\todo{Mention that we maximize the union of sets $S_{ef}$, without considering the gain in the \MCI objective function if two edges of different sets are used (this will be taken into account in the $1/k-1$)}
  \item Return all corresponding edges: $SOL = \cup_{i=1}^{k/2} \{e_i, f_i\}$. Please note that $SOL$ maybe contain less than $k$ elements.
\end{enumerate}

We now have the following: 
$$|S_{SOL}| \geq |\cup_{(e, f) \in P} S_{ef}| \enspace .$$

Let $OPT$ be the solution for the MCI instance with input $k$ and $v$ and let $M$ be the set consisting of the $k/2$ elements from $OPT \times OPT$ with a union of maximum cardinality:

$$M = \argmax_{X \subset OPT \times OPT, |X| = k/2} |\cup_{(e, f) \in X} S_{ef}| \enspace .$$

We have used the greedy algorithm for maximum coverage:
$$|\cup_{(e, f) \in P} S_{ef}| \geq \left(1-\frac{1}{e}\right)|\cup_{(e, f) \in M} S_{ef}| \enspace .$$

If there is a member in $S_{OPT}$, then a corresponding shortest path will use two edges in $OPT$:
$$S_{OPT} = \cup_{(e, f) \in OPT \times OPT} S_{ef} \enspace .$$

The set $S_{OPT}$ is a union of ${k \choose 2}$ sets and $\cup_{(e, f) \in M} S_{ef}$ is the union of $k/2$ of these sets with maximum cardinality, so we can use Lemma~\ref{lem:union_x_y_z}:
$$|\cup_{(e, f) \in M} S_{ef}| \geq \frac{k/2}{{k \choose 2}} |S_{OPT}| = \frac{1}{{k-1}} |S_{OPT}| \enspace .$$\todo{If we add $\beta$ more edges, we have $\geq\frac{\beta}{{k-1}}|S_{OPT}|$? Martin: I think that is correct but the argument requires $\beta \leq k-1$ (I think).}

Now we can put it all together:
$$|S_{SOL}| \geq \left(\left(1-\frac{1}{e}\right)/(k-1)\right) |S_{OPT}| \enspace .$$

The approach can maybe be extended from choosing pairs to triples, etc.

